Accelerating Hessian-free optimization for deep neural networks by implicit preconditioning and sampling

Hessian-free training has become a popular parallel second or- der optimization technique for Deep Neural Network training. This study aims at speeding up Hessian-free training, both by means of decreasing the amount of data used for training, as well as through reduction of the number of Krylov subspace solver iterations used for implicit estimation of the Hessian. In this paper, we develop an L-BFGS based preconditioning scheme that avoids the need to access the Hessian explicitly. Since L-BFGS cannot be regarded as a fixed-point iteration, we further propose the employment of flexible Krylov subspace solvers that retain the desired theoretical convergence guarantees of their conventional counterparts. Second, we propose a new sampling algorithm, which geometrically increases the amount of data utilized for gradient and Krylov subspace iteration calculations. On a 50-hr English Broadcast News task, we find that these methodologies provide roughly a 1.5x speed-up, whereas, on a 300-hr Switchboard task, these techniques provide over a 2.3x speedup, with no loss in WER. These results suggest that even further speed-up is expected, as problems scale and complexity grows.

==> introOld.tex <==
\section{Introduction}
Second order and super-linear optimization techniques have been extensively explored for problems involving pathological curvature, such as deep neural network (DNN) training problems. In fact, \cite{Martens2010} demonstrated success of a second order technique, known as Hessian-free optimization \cite{ Horesh2006}, with DNNs on various image recognition tasks. In addition \cite{bedk:hf}, successfully applied the Hessian-free optimization technique with DNNs for speech recognition tasks. Other super-linear methods, including L-BFGS \cite{google:dist} and Krylov Subspace Descent \cite{povey:kyrlov}, have also shown great success for DNN training. 

%While some of the aforementioned methods are regarded in the literature as second order methods, in practice, in their inexact forms \footnote{Here inexactness relates to approximation of the Hessian (or its action upon vectors) to a finite level of precision. The level of precision is typically associated with the computational budget allocated for the task. At the limit, most methods asymptotically converge to the true Hessian} and for residuals that are not small, these methods exhibit super-linear convergence. For the sake of correctness, henceforth we shall denote them as such. 

Super-linear methods are particularly important for sequence-training of DNNs. Sequence-training has been shown to provide a relative improvement between 10-20\% in WER over a cross-entropy trained DNN \cite{bedk:nn}. Because sequence training must use information from time-sequential lattices corresponding to utterances in the training data, sequence training is performed using utterance randomization rather than frame randomization. For mini-batch stochastic gradient descent, which is often used for cross-entropy training, frame randomization seems to perform better than utterance randomization \cite{seide:sequence}. However, because sequence-training must be accomplished at the utterance level, super-linear methods outperform much better than SGD, as second order methods compute the gradient over a large batch of utterances compared to utterance mini-batch based SGD which computes the gradient over just one utterance \cite{bedk:hf}. 

At IBM Research, we employ Hessian-free optimization techniques for sequence training \cite{Martens2010}. One of the drawbacks of this method is that training can be very slow, requiring about 3 weeks of training for a 300-hour Switchboard task \cite{bedk:hf}. There are two reasons why training is slow. Firstly, a great number of Krylov subspace iterations (depending upon the Hessian’s spectrum), may be required for solution of the normal system of equations (i.e. approximating the Hessian), within each non-linear optimization iteration \cite{Martens2010}, \cite{bedk:hf}. Secondly, \cite{bedk:hf} proposes using a fixed amount of data for all HF iterations in both the gradient and Krylov subspace iteration computations. The purpose of this research is to explore algorithmic strategies for reduction of the amount of time spent in both gradient and Krylov subspace computations, both by reducing the amount of data need to be accessed and transferred for training, as well as by reducing Krylov subspace iteration count consumed for estimating the Hessian.

Preconditioning in the context of linear algebra refers to the process of transforming a system of equations into one that can be solved more readily \cite{templates1994}. For example, pre-conditioning has been extensively used to reduce iteration count of Krylov subspace iterative schemes \cite{eisenstat:preconditioning}. Obtaining an appropriate pre-conditioner for a given problem can be challenging \cite{chapelle:jacobi}. 
% For example, we have found this to be the case with the Jacobi pre-conditioner %\cite{chapelle:jacobi}.
First, since the spectral characteristics of each domain problem are problem-specific. Second, while in principle, it is possible to design preconditioning strategies that will reduce the computational burden of the consequent solution phase radically (e.g. preconditioner that completely invert a matrix), yet, the computational investment in attainment and application of such preconditioning scheme might offset the benefit of their use. Thus, it is critical to identify a proper balance between computational efforts invested in preconditioning, vs. that invested in the consequent solution phase. 
%It is important to note here, that not all, pre-conditioning schemes provide fine-level (if at all) means for controlling preconditioning extent. Third, most preconditioning strategies relies upon explicit access to the underlying matrix. Thus, despite its potential impact for large-scale problems and due to its complexity, preconditioning of implicit systems has remained vastly under-researched. 

% if the pre-conditioning process is computationally expensive to obtain, then this will offset any reduction in conjugate gradient iterations, and thus the pre-conditioner will not be effective. 

For our optimization problem, it is computationally intractable to construct the Hessian explicitly. This fact renders decomposition and multi-grid based preconditioning methods impractical. Quasi-Newton approaches were originally designed for solution of non-linear optimization problems. These approaches, construct (typically a low rank) approximation to the Hessian, and in their limited memory versions, only form such approximations implicitly. In this work, we propose the application of quasi-Newton L-BFGS method \cite{nocedal:lbfgs} as a pre-conditioner for solution of the linear systems of equations by flexible Conjugated Gradients. At the limit of constraining the Krylov subspace iteration to 0, the approach is equivalent to a plain vanilla quasi-Newton solution of the non-linear problem, yet, as our results indicate, the use of quasi-Newton methods as pre-conditioner can be extremely effective. The rationale is that both quasi Newton approaches and Krylov subspace methods, exploit the underlying structure of the linear(ized) system. Nonetheless, the postulated structural assumptions of both (low rank, Krylov subspace) are complementary, thus, a proper combination of which is typically more effective than dependence upon each one solely.  

The use of an L-BFGS scheme for pre-conditioning has been suggested before \cite{morales:lbfgs} for numerical simulations. We extend upon the work in \cite{morales:lbfgs}, and demonstrate that L-BFGS serves as an effective pre-conditioner for Krylov subspace based Hessian free training of DNNs on large-scale speech recognition data. Furthermore, unlike \cite{morales:lbfgs} which used a typical fixed CG approach, we make here an important observation that non-fixed point preconditioners, as the proposed L-BFGS, cannot be used stably with standard Krylov subspace iterative schemes\cite{ templates1994}. Thus, to ensure, stable and predictable convergence, we propose here the use of flexible variants of Krylov subspace methods. These variants avoid the failures and breakdowns that their standard counterparts are susceptible to.
 
Second, we introduce a sampling strategy in which the amount of data used for gradient and Krylov subspace iteration calculations, is geometrically increased. The use of incremental sample size has become common in gradient estimation. The general idea is to gradually include additional training examples out of the complete set of training samples, and thereby attain gradient estimate of desirable levels of fidelity. These methods often decrease the objective function loss quickly during initial training iterations, albeit, during later iterations the sampling process tends to significantly slows down progress. On the other end of the spectrum, full gradient methods compute the gradient on all of the data. While this computation is expensive, they achieve much better convergence of the objective function. In this study, we propose a hybrid method that captures the benefits of both incremental and full gradient methods, by increasing the amount of sampled data used for gradient and Krylov subspace iteration calculations. 
\cite{FriedlanderSchmidt2012} explored first and second order hybrid methods that gradually increase the amount of data as the algorithm proceeds, and provided theoretical results linking convergence rates to sampling errors. 
Sampling the amount of data used for gradient and Krylov subspace calculations for second order methods was also explored in \cite{Byrd2012}, who observed the variance of the batch gradient in order to determine the amount of data to use for gradient and Krylov subspace calculations on subsequent iterations. However, this approach requires calculating the variance of the gradient estimate, which requires two passes through the network. We will show experimentally the drawbacks of this approach for speech recognition in the Numerical Results section. \cite{FriedlanderSchmidt2012} explored a simple geometric sampling strategy; geometrically increasing the amount of data used for logistic regression and conditional random field (CRF) problems. 
This strategy was further analyzed and used for large-scale inverse problems in~\cite{AravkinFHV:2012}. 
The benefit of this approach is that the schedule for selecting data is given ahead of time, and there is no need to compute the computationally expensive gradient variance. In this paper, we extend the idea in \cite{FriedlanderSchmidt2012} for DNN problems.

Initial experiments were conducted on a 50-hr English Broadcast News (BN) task \cite{bedk:hf}. We find that pre-conditioning allows for more than 20\% speedup by reducing the number of Krylov subspace iterations. Furthermore, we find that gradient and Krylov subspace sampling provide roughly additional 20\% improvement in training time. In total, by combining both sampling and pre-conditioning speedup ideas we were able to reduce overall training time by a factor of 1.5. Second, we extend the preconditioning and sampling ideas to a larger 300-hr Switchboard (SWB) task, where we find that the proposed techniques provide more than a 2.3x speedup.

The remainder of this publication is organized as follows. The Hessian-free algorithm utilized in this paper is described in Section 2. Implicit pre-conditioning is discussed in Section 3, while gradient sampling is presented in Section 4. Experiments and results using the proposed methods are elucidated in Sections 5 and 6 respectively. Finally, Section 7 concludes the study.
%
%We propose a methodology of applying an L-BFGS pre-conditioner to the conjugate gradient component of the Hessian-free optimization training for DBNs. The advantages of this pre-conditioner are as follows:
% \begin{enumerate}
% \item The pre-conditioner reduces the number of CG iterations significantly
% \item The pre-conditioner is cheap to obtain, and therefore does not significantly impact overall CG time
% \item The pre-conditioner allows for roughly a 22\% speedup in overall training time.
% \end{enumerate}
 
%Hessian-free strategy has become a popular parallel super-linear optimization technique for Deep Neural Network training. This study aims at speeding up Hessian-free training, both by means of decreasing the amount of data used for training, as well as through reduction of the number of Krylov subspace solver iterations used for implicit estimation of the Hessian. The main bottleneck of Hessian free strategies is the excessively large number of Krylov subspace iterations needed to be solved per single non-linear iteration. Typically, this iteration count can be radically reduced by means of preconditioning, however, most preconditioning schemes, requires explicit access to the matrix (Hessian in our case) under consideration. In this study, we developed an L-BFGS based preconditioning scheme that avoids the need to access the Hessian explicitly. Since L-BFGS cannot be regarded as a fixed-point iteration, we further propose here the employment of flexible Krylov subspace solvers that retain the desired theoretical convergence guarantees of their conventional counterparts. Second, we propose a new sampling algorithm, in which geometrically increasing the amount of data are utilized for gradient and Krylov subspace iteration calculations. On a 50-hr English Broadcast News task, we find that these methodologies provide roughly a 1.5x speed-up, whereas, on a 300-hr Switchboard task, these techniques provide over a 2.3x speedup. These results, suggest that even further speed up is expected, as problem scale and complexity grows larger.
 


